Articulation rate in Swedish child-directed speech increases as a function of the age of the child even when surprisal is controlled for

In earlier work, we have shown that articulation rate in Swedish child-directed speech (CDS) increases as a function of the age of the child, even when utterance length and differences in articulation rate between subjects are controlled for. In this paper we show on utterance level in spontaneous Swedish speech that i) for the youngest children, articulation rate in CDS is lower than in adult-directed speech (ADS), ii) there is a significant negative correlation between articulation rate and surprisal (the negative log probability) in ADS, and iii) the increase in articulation rate in Swedish CDS as a function of the age of the child holds, even when surprisal along with utterance length and differences in articulation rate between speakers are controlled for. These results indicate that adults adjust their articulation rate to make it fit the linguistic capacity of the child.

==> README <==
____________________
The HYPHENAT package

    The hyphenat package can be used to disable all hyphenation
in a document or in selected text within the document. It also 
enables hyphenation within `words' that contain analphabetic 
characters (e.g., that include underscores), and hyphenation of
text typeset in monospaced (e.g., CM typewriter) fonts.


______________
Change history

Version 2.3c
- New maintainer (Will Robertson)

Version 2.3a
- Fixed a double hyphenation problem with some non-CM fonts.

Version 2.3
- Added \hyp command for hyphenation of compound hyphenated words.

----------------------------------------------------------------- 
  Author: Peter Wilson, Herries Press
  Maintainer: Will Robertson (will dot robertson at latex-project dot org)
  Copyright 1998--2004 Peter R. Wilson
 
  This work may be distributed and/or modified under the
  conditions of the LaTeX Project Public License, either
  version 1.3c of this license or (at your option) any 
  later version: <http://www.latex-project.org/lppl.txt>

  This work has the LPPL maintenance status "maintained".
  The Current Maintainer of this work is Will Robertson.
 
  This work consists of the files:
README (this file)
hyphenat.dtx
hyphenat.ins
hyphenat.pdf (user manual)
  and the derived files:
hyphenat.sty

    The distribution consists of the following files:
README (this file)
hyphenat.ins
hyphenat.dtx
hyphenat.pdf

----------------------------------------------------------------- 

    To install the package:
- run: latex hyphenat.ins (which will generate hyphenat.sty)
- Move hyphenat.sty to a location where LaTeX will find it
  (typically in a local texmf tree at tex/latex/hyphenat) and refresh the
  file database. See the FAQ on CTAN at help/uk-tex-faq or
  http://www.tug.ac.uk/faq for more information on this.

    To process the user manual:
- run: latex hyphenat.dtx
- (for an index run: makeindex -s gind.ist hyphenat)
- run: latex hyphenat.dtx
- Print hyphenat.dvi for a hardcopy of the package manual 

2004/04/22
Peter Wilson

